Incivility in Open Source Projects: A Comprehensive Annotated Dataset of Locked GitHub Issue Threads

In the dynamic landscape of open source software (OSS) development, understanding and addressing incivility within issue discussions is crucial for fostering healthy and productive collaborations. This paper presents a curated dataset of 404 locked GitHub issue discussion threads and 5961 individual comments, collected from 213 OSS projects. We annotated the comments with various categories of incivility using Tone Bearing Discussion Features (TBDFs), and, for each issue thread, we annotated the triggers, targets, and consequences of incivility. We observed that Bitter frustration, Impatience, and Mocking are the most prevalent TBDFs exhibited in our dataset. The most common triggers, targets, and consequences of incivility include Failed use of tool/code or error messages, People, and Discontinued further discussion, respectively. This dataset can serve as a valuable resource for analyzing incivility in OSS and improving automated tools to detect and mitigate such behavior.

==> sections/conclusion.tex <==
\section{Conclusion}
This paper offers a comprehensive exploration of incivility within open-source software (OSS) development, by presenting a carefully curated dataset of 400 locked issue threads from 220 substantial OSS projects. The analysis, encompassing 5395 comments annotated with uncivil Tone Bearing Discussion Features (TBDFs), reveals prominent features, triggers, targets, and consequences of incivility within these discussions. 
Notably, \textit{Bitter frustration}, \textit{Impatience}, and \textit{Mocking} emerge as the most prevalent uncivil features, shedding light on the diverse tones and expressions present in OSS issue threads. 
The abundance of triggers such as \textit{Failed use of tool/code or error messages}, \textit{Technical Disagreement}, and \textit{Communication Breakdown}, alongside a diverse array of targets such as \textit{People}, \textit{Code/tool}, and \textit{Company/organization}, coupled with consequences like \textit{Discontinued further discussion}, \textit{Escalating further}, and \textit{Provided technical explanation}, illuminates the intricate and multifaceted nature of incivility dynamics within these OSS projects. 
This dataset can help foster healthier and more constructive collaborations within the OSS community. Future research can build upon these findings, delving deeper into the contextual nuances of incivility and exploring tailored interventions to promote positive interactions in open-source development.

==> sections/limitations.tex <==
\section{Limitations and Future Improvements}

